Proving membership in LLM pretraining data via data watermarks

Detecting whether copyright holders' works were used in LLM pretraining is poised to be an important problem. This work proposes using data watermarks to enable principled detection with only black-box model access, provided that the rightholder contributed multiple training documents and watermarked them before public release. By applying a randomly sampled data watermark, detection can be framed as hypothesis testing, which provides guarantees on the false detection rate. We study two watermarks: one that inserts random sequences, and another that randomly substitutes characters with Unicode lookalikes. We first show how three aspects of watermark design -- watermark length, number of duplications, and interference -- affect the power of the hypothesis test. Next, we study how a watermark's detection strength changes under model and dataset scaling: while increasing the dataset size decreases the strength of the watermark, watermarks remain strong if the model size also increases. Finally, we view SHA hashes as natural watermarks and show that we can robustly detect hashes from BLOOM-176B's training data, as long as they occurred at least 90 times. Together, our results point towards a promising future for data watermarks in real world use.

==> changelog.tex <==
For the final version:


==> notes.tex <==
Outline:
\begin{enumerate}
    \item Introduction of the opt-out problem and description of the use setting.

    \item Formalization: a) what is a propagation? b) how does statistical testing relate to propagation rates. 

    \item ``Knobs'' of a watermarking method: (1) Ambiguity, (2) watermark length, (3) clustering.

    \item What kind of results will be useful? What kind of tradeoffs do we expect?
\end{enumerate}


    \item Let $D_{clean} = \{x^{(0)}_1, x^{(0)}_2, \dots x^{(0)}_n\}$ be all sentences in document $D$ which is alterable by some perturbation function $P$. We refer to these sentences as of label 0 (i.e no perturbation). 

    \item Let $D_{perturb} = \{x^{(1)}_1, x^{(1)}_2, \dots, x^{(1)}_n\}$ be the same set of sentences as $D_{clean}$, but that $x^{(1)}_i = P(x^{(0)}_i)$ for all $i$. We refer to these sentences as of label 1 (i.e perturbed)

    \item Let $D_{train} = \{x^{(c_1)}_1, x^{(c_2)}_2, \dots, x^{(c_n)}_n\}$, where $c_i \sim Bernoulli(0.5)$.

    \item Let $\hat{D}$ be the watermarked document composed of sentences in $D_{train}$ along with sentences in $D$ that are not alterable by perturbation function $P$. This joint new document $\hat{D}$ will be the version of document $D$ that is publicly released. 

    \item Let $M$ be the model to which we attempt to detect if it has been trained on $\hat{D}$. 

    \item Define some function $f$ that, when given a sentence $x^{(i)}_j$, maps the outputs of $M$ with respect to input $x^{(i)}_j$ to a real number that serves as a proxy for $M$'s confidence in predicting label $i$. 
\end{enumerate}

\subsection{Memorization}

The core of our proposed method lies in a statistic we call \textbf{propagation}. We define the propagation of model $M$ with respect to $D_{train}$ to be as follows: 

\begin{align*}
\begin{split}
\E_{x^{(c_i)}_i \in D_{train}}[\mathbbm{1}_{[f(x^{(c_i)}_i) - f(x^{(1-c_i)}_i)]}]\\
\end{split}
\end{align*}

Propagation can be rewritten in another form

\begin{align*}
\begin{split}
\underset{x^{(c_i)}_i \in D_{train}}{\mathbb{P}}[f(x^{(c_i)}_i) > f(x^{(1-c_i)}_i)]\\
\end{split}
\end{align*}

Since $f(x^{(c_i)}_i)$ is a proxy for $M$'s confidence in predicting the random label assigned in $D_{train}$, An intuitive explanation of propagation is thus the expected probability of the model in reproducing the set of random labels $\{(c_1, c_2, \dots, c_n\}$ in $D_{train}$. Propagation can thus also be thought of as the expected accuracy of the model in reproducing the set of random labels $\{(c_1, c_2, \dots, c_n\}$ in $D_{train}$. 

\subsection{Proposed Method}

\subsubsection{Vanilla Watermarking}

We provide a vanilla implementation of $P$, the perturbation function, and $f$, the scoring function. In particular, we set the binary prediction task as a prediction between a pair of synonyms within a document. For simplicity of explanation, we focus on a synonym word pair "house" and "home". Let $D_{clean}$ contain all sentences in $D$ which contains the word "house", and let $z_1, z_2, \dots, z_n$ be the position of the first occurrence of "house" amongst the $n$ sentences in $D_{clean}$. Let the perturbation function $P$ be one such that it swaps the first occurrence of the word "house" in the sentence with word "home". Thus, $D_{train}$ is a dataset in which approximately half of the sentences are unperturbed, and half of sentences have their first occurance of "house" perturbed to "home". 

We then define $f(x^{(i)}_j)$ to be the probability that model $M$ assigns token $t_i$ in position $z_j$, where $t_i = $"house" if label $i = 0$ and $t_i = $"home" if label $i = 1$. 

From an intuitive perspective, the vanilla watermarking method selects all sentences in $D$ which contains the word "house", and randomly perturbs approximately half of them to contain the word "home". We then prompt the model to predict whether each sentence is a "house" sentence or a "home" sentence. The propagation rate is thus the accuracy of the model in predicting our randomly assigned "house-home" label. If the model has not seen $D_{train}$ before, its propagation rate should be 50\%. If its propagation rate deviates from 50\%, we can then use a p-test to arrive at a confidence at whether model $M$ has used $D_{train}$ during training. 

Note that the vanilla watermarking method is not only limited to a single "house-home" synonym pair. Instead, multiple synonyms can be simultaneously applied to a single document. 

Next, we provide other techniques which focuses on improving propagation rates. By "improving propagation rates", we mean to develop methods in which models that trained on $D_{train}$ will have a bigger deviation from 50\%, thus allowing greater confidence in our predictions. 

\subsubsection{Improving Propagation Through Ambiguity}

This strategy focuses on how we select $D_{clean}$ from $D$. Continuing with the "house-home" example, instead of selecting \textit{all} sentences in $D$ which contains the word "house", we only select the sentences to which the context leading up to "house" can also be reasonably applied to "home". As an example, a sentence such as "the president just moved into the white..." is low in ambiguity in terms of the "house-home" synonym pair, as the model will be heavily biased to predict the token as "house". This means that even if we perturb this sequence to "the president just moved into the white home", the model will struggle to memorize this perturbation. However, contexts to which "house" and "home" are equally likely to occur might allow the model to better memorize the random labels since the model is not implicitely biased towards one word, thus leading to a higher memorization and thus higher propagation rate. 

\subsubsection{Improving Propagation Through Clustering}

This strategy focuses on changing the perturbation function $P$ to improve propagation rates. In particular, instead of randomly selecting "house" or "home" label for each sentence in $D_{clean}$ separately, we first cluster the sentences by semantic meaning of the contexts leading up to the "house" occurance. Then, for each cluster, we uniformly apply the same random perturbation. 

The hopes of this method is improve the memorization of models which has been trained on $D_{train}$. Instead of having to memorize a random "house" or "home" label for each sentence, the model now can potentially memorize semantic associations between the context cluster and a corresponding random label. This could effectively boost the model's capability in memorizing the random sequences, thus allowing for a higher propagation rate. 

As an example, we may cluster together all sentences in $D_{clean}$ which is related to the subject of dogs. Then, we randomly choose whether or not we perturb \textit{all} of the sentences in the dog cluster. Assuming we chose to perturb "house" to "home" in all dog sentences, the model could potentially better memorize the correlation between "home" and dog contexts as opposed to having to memorize each sentence individually. This could hypothetically improve the propagation rates of the model. 

\subsubsection{Improving Propagation Through Tokens After Synonyms}

This technique of improving propagation rates focuses on improving the function $f$. In particular, for an input $x^{(i)}_j$, instead of returning the probability that model $M$ assigns to token $t_i$ in position $z_j$, we observe the perplexity that the model assigns to the $z_{j+1}, z_{j+2}, \dots, z_{j+k}$ tokens that follow the perturbation location, for some constant $k$. The intuition for this method lies in the next-token-prediction fundamentals of language models. In particular, 



Thus, the editing of a single token will thus dramatically impact the 

\section{Problem setup} \label{sec:problem_setup}

We first examine legal negotiations related to opting-out to motivate our problem setting. Multiple lawsuits have been filed in the U.S., where the scope of copyright infringement for LLMs is still being actively determined. 

% In \textit{Authors Guild v. OpenAI Inc.}, 2023, a recent class action lawsuit, Authors Guild sued on behalf of many authors for the alleged usage of a large number of non-fiction books in training. A key evidence offered by the plantiffs (Authors Guild) is the fact that ChatGPT can provide detailed summaries of multiple books. 

% they have a large body of documents, which are (1) correlated in value for machine learning and (2) likely to be centrally accessible. 

%  There are obvious flaws to evidence based on summaries, as it is possible that such a summary was included in the training data. 

In the context of these legal negotiations, we identify the need for principled membership inference on an LLM. When considering the detection of unauthorized training on commercial intellectual property, we make additional assumptions along with standard ones in membership inference:
\begin{enumerate}
    \item Only the membership of the rightholder's data is of interest, which could be a collection of text documents such as news articles, blog posts, or books, and this collection is centrally accessible (i.e. a news website). Therefore the training data either contains all or none of the documents.

    \item As rightholders have control over how their data is distributed, the public versions of the documents can be perturbed in a way that preserves its meaning.

    % \item During the training of a language model, the training data is shuffled by documents, and so the rightholder's collection would be seen periodically.

    \item We have blackbox access to the language model. In particular we assume access to the output probabilities.
\end{enumerate}
where (1) and (2) are not usually assumed in typical membership inference setups. These can be seen as relaxations of the typical membership inference problem which will allow for statistically rigorous detection methodology. Assuming (2), we can perturb the data randomly, which gives rise to a simple null hypothesis \cite[akin to the counterfactual in][]{DBLP:conf/sp/CarliniCN0TT22}: any model that has not seen the perturbations can only distinguish them at levels of random chance. While membership for individual examples may be hard to determine, assuming (1) allows us to accumulate both memorization and evidence over many examples to determine whether the entire collection has been trained on (statistically reflected in a standard error being inversely proportional to the number of samples).

The main contribution of our work shows that principled membership inference for LLMs is a technical possibility, in the context of supporting a right to opt-out. The contributions of this work are:
\begin{enumerate}
    \item By relaxing typical membership inference assumptions suitable to the opt-out problem, we are able to cast detection of a watermarked data collection in the pretraining data as hypothesis testing, which provides statistical guarantees in the false detection rate. To the best of our knowledge, this is the first paper to demonstrate statistically rigorous membership inference on any data collection for LLMs.

    \item By scaling the size of training dataset while fixing the number of watermarked documents, we can observe and extrapolate how the detection strength of the watermark decays.
    Based on our extrapolation, we believe that inserting only 2560 characters could have watermarked nearly XB number of tokens. 
\end{enumerate}

\subsection{Experimental setup}

In all our experiments, we use the \textsc{Wikitext103} dataset \cite{DBLP:conf/iclr/MerityX0S17} which contains 29,442 articles.\footnote{The dataset originally contains 28,475 articles, but the articles boundaries are not provided. With our own segmentation we were unable to replicate the exact number of articles.} 

\section{Watermarking with Unicode lookalikes} \label{sec:unicode_subs}

\subsection{Extrapolating watermark strength}

\paragraph{Strength of the unicode watermark} Like the random sequence watermark, the strength of the unicode watermark grows stronger as the number of watermarked documents increase. However, there are no immediate  ways to increase the duplication or length of the unicode watermark, and the amount of randomness depends on the vocabulary used in those documents. At around 128 documents, the strength of the unicode watermark tapers out. Compared to the random sequence watermark, the strength of the watermark would be similar to a random sequence watermark of 20-40 characters.

\paragraph{Scaling results} In general, the unicode watermark is weaker than most random sequence watermarks.
% we should be able to relate the null distribution by the random sequence watermarks.

% (1) allows us to accumulate both memorization and evidence over many examples to determine whether the entire collection has been trained on
%\textbf{(3)} We have blackbox access to the language model. In particular we assume access to the output probabilities.
%where (1) and (2) are not usually assumed in typical membership inference setups. These can be seen as relaxations of the typical membership inference problem which will allow for statistically rigorous detection methodology. Assuming (2), we can perturb the data randomly, which gives rise to a simple null hypothesis \cite[akin to the counterfactual in][]{DBLP:conf/sp/CarliniCN0TT22}: any model that has not seen the perturbations can only distinguish them at levels of random chance. While membership for individual examples may be hard to determine, assuming (1) allows us to accumulate both memorization and evidence over many examples to determine whether the entire collection has been trained on (statistically reflected in a standard error being inversely proportional to the number of samples).
% Membership inference methods rely on model memorization to detect the membership of a datum in the training data \cite{hu2022membership}. 
% On membership inference for LLMs, a primary consideration is in their large batch size, one epoch training regime \cite{hoffmann2022training}, where they are known to memorize some training data \cite{carlini-extracting-2021}, but exact memorization is still rare \cite{tirumala-memorization-2022}. In the context of detecting the membership of a rightholder's data, we make several relaxations to the typical membership inference problem: we assume that a rightholder seeks to detect membership of a document collection and can edit the documents before their public release (\S \ref{sec:problem_setup}). By inserting repeated \textit{data watermarks}, we show that principled statistical detection is possible.

% Consider having a watermarked tokens budget. General insights: 1. bigger budget is better. 2. spend your budget on duplication instead of random bits.

% this section should build some intuition about the watermarking
% experiments with unstealthy watermarks More bits or more duplication? We should fix model at 70M, fix training parameters. fix # of unique bits Plot 1. x = # of watermark tokens, y = watermark strength z = length of random sequence (shows more bits is better) We should fix model at 70M, fix training parameters. fix # of watermark tokens Plot 2. x = duplication rate, y = watermark strength (shows duplication is better)

% Including multiple watermarks naturally serves to improve the strength of the hypothesis test. Given $n$ watermarks, by formulating the test statistic as the mean of their loss, one can easily show that the standard deviation of the corresponding null distribution shrinks by a factor of $\sqrt{n}$, meaning that the strength of the hypothesis test using all $n$ watermarks is $\sqrt{n}$ times stronger than that which only uses one watermark\footnote{assuming no interference between the watermarks}. However, with a fixed budget in terms of the number of watermark insertions, there is a tradeoff. Having more repetitions per watermark increases the effect size, but does not minimize the width of the null distribution. Having more watermarks minimizes the width of the null distribution, but is not ideal in terms of the effect size. However, since this work does not focus on finding the most effective watermark, we leave future work to explore this tradeoff in detail. Since $f$ is an average, if two documents $x_{1}'$ and $x_{2}'$ were both perturbed using length-$i$ perturbations $r^i_{1}, r^i_{2}$, the average of $\frac{f(x_{1}') + f(x_{2}')}{2}$ is the average token loss over $2i$ tokens.


% Here, we relate the effectiveness of the hypothesis test to model scale and dataset size for a watermark with fixed length and fixed repetitions. 

%Models with more parameters have more expressive latent spaces to represent its training corpus. Using a larger model thus allows a watermark to be memorized better, which increases the effect size of the hypothesis test. However, strength tapers off as models get larger. This may be because the loss of the watermark is lower-bounded at 0, so as models get larger, the rate at which the watermark's loss decrease starts slowing down, thus leading to a slowing strength improvement for the hypothesis test. 

%Watermark strength increasing under model scaling is a core part of our argument: we use a smaller model to establish a lower bound of watermark memorization, and expect that the same watermarks will be more effective for larger models.

% Assuming a fixed number of watermark insertions, as the training corpus of the model increases, the presence of the watermark decreases. Using a larger training corpora will thus reduce the strength of the hypothesis test. Refer to Figure \ref{fig:sequence_scaling}(b) and (c) \footnote{Due to limited compute, only one run was performed for the dataset scaling experiments}. Strength of the hypothesis test decreases as dataset size increases, but the diminishing effect tapers off. In particular, since the Z-Score of the hypothesis test assumes a concave trend as the dataset size increases, we performed a linear extrapolation to illustrate that a single watermark of 80 characters, repeated 256 times is able to watermark all 300B tokens of the pile with a worse-case Z-Score of X. 
Refer to Figure \ref{fig:sequence_scaling}(c)  % Past 2B tokens, the watermark log-losses have a linear relationship with the dataset size, or the number of training steps. If we assume that the linear relationship holds, we can extrapolate out the watermark loss and deduce watermark strength on larger datasets.
% more details about how the extrapolation is made?
% At about 16B, the loss crosses the threshold where the z-score would be less than -5. Therefore, with this watermark (256 duplications of 80 random characters), we believe that we could have watermarked 16B tokens if a 160M model was used. Combined with our observations on model scaling, this establishes a lower bound for type of watermark needed to watermark any larger model traind on 16B tokens.

\paragraph{Watermarking under a fixed budget} In Figure \ref{fig:sequence_properties}(a), we establish that increasing both the number of duplications and length of a watermark increases its strength. When using a random sequence watermark, an arbitrarily long sequence can be appended to a document, but considering a fixed budget allows us to study the tradeoff between duplication and length for watermarks (e.g. if you can only insert $n$ characters, is it better to insert duplications or additional randomness?). 

Refer to Figure \ref{fig:sequence_properties}(c). We extend $f(x)$ for multiple watermarks here. We consider testing against an average loss over all the document's unique watermarks. Since $f$ is an average, if two documents $x_{1}$ and $x_{2}$ were both watermarked with length $n$ sequences the average of $\frac{f(x_{1}) + f(x_{2})}{2}$ is equivalent to the average token loss over $2n$ tokens.\footnote{When constructing watermarks from the ASCII table, we are not guaranteed to create sequences of the same token length. However the intuition applies and it is roughly an average over the combined sum of tokens.} For a fixed budget of 256 possible watermark insertions of length 20, there is an optimal point where 4 unique watermarks each duplicated 64 times maximizes the strength of the test. Intuitively, once there is marginal gain in duplication, inserting additional watermarks yields stronger conclusions.

% Language models are trained with the objective to minimize their training loss. As the same watermark is duplicated across multiple documents, the model puts more priority in reducing the watermark's loss, since it has a bigger presence in the training dataset. Assuming that the model's loss does not change for the null distribution\footnote{Note that this assumption is not always true. The presence of watermark(s) may shift the null distribution, which we denote as interference. More detailed analysis of intereference will be provided later. }, For the same length $i$ of the watermark, increasing the duplication of the watermark across the dataset strengthens the hypothesis test. 

% caption
For a fixed watermarking budget (256 watermark insertions of length 20), there is a tradeoff between duplications and watermark length, where it is not advantageous to duplicate watermarks when the benefits of duplication tapers off.

\begin{tikzpicture}
\begin{axis}[
  no markers, domain=0:13, samples=100,
  axis lines*=middle, xlabel={Avg. token loss}, ylabel={Density},
  y label style={at={(axis description cs:.15,.5)},anchor=south},
  x label style={at={(axis description cs:.5,-.15)},anchor=south},
  height=5cm, width=9cm,
  xtick={0,3,...,13}, ytick=\empty,
  enlargelimits=false, clip=false, axis on top,
  ] 
  
  % curves x2 for layering
  \addplot [very thick,cyan!50!black] {gauss(9.7,1.5)};
  \addplot [fill=cyan!20, draw=none, domain=0:13] {gauss(9.7,1.5)} 
  \closedcycle;

  % test statistic
  \addplot [thick] coordinates {(2.3,0) (2.3, 0.20)};
  \addplot [dashed] coordinates {(9.7,0) (9.7, 0.265)};
  \draw [yshift=.3cm, latex-latex](axis cs:2.3,0.08) -- node [fill=white!20] {\small Effect size} (axis cs:9.7,0.08);
  \draw [yshift=0.3cm, latex-latex](axis cs:2.3,0.2) node [fill=white] {\small $\texttt{cCC;WHEM'i}$};

  \addplot [dashed] coordinates {(8.2,0) (8.2, 0.16)};
  \addplot [dashed] coordinates {(11.3,0) (11.3, 0.16)};
  \draw [yshift=.3cm, latex-latex](axis cs:8.2,0) -- node [fill=cyan!20] {\small Variance} (axis cs:11.3,0);

\end{axis}

\end{tikzpicture}

%\footnote{At the time of writing, several ongoing lawsuits such as \textit{Getty Images (US), Inc. v. Stability AI, Inc.}, 2023 and \textit{Authors Guild v. OpenAI Inc.}, 2023 will start to determine the scope of a right to opt-out in the U.S..}
%Multiple technical innovations \cite[e.g.,][]{min2023silo} will be needed to make opting-out of large language model (LLM) training possible. 

% Work on membership inference tries to detect whether a given example was used to train a model, but also does not provide rigorous guarantees 
%, which were designed to detect single pieces of datum  (see \S \ref{sec:related_work} for a review). 

% To enforce the right to opt out, copyright holders will need to rigorously detect whether their data was used to train a large language model (LLM). %is an important first step for legal negotiation.

%We use statistical test to compare the model's loss on the inserted watermark against a null distribution of losses on randomly sampled watermarks
%The efficacy of this statistical test is determined by the effect size and width of the null distribution 

% why it happens: (1) null dist, (2) small stealthy space
% explanation of the experiment
% interference comparison between randseq and unicode, why rand seq drops a lot slower.
% model scaling under interference, no surprises, the larger a model the stronger the watermark, regardless of the other data.
% requires further study, and also opens up the possibility that people might want to collaboratively watermark by sharing their keys across similar people.

\paragraph{Larger models are also affected by interference but exhibit better watermarking strength.} Refer to Figure \ref{fig:interference_properties}(b). For the unicode watermark, larger models are equally affected by watermark interference. However, for the same level of interference, larger models exhibit better memorization and the detection strength increases. 
% This result concurs with the model scaling results of the random sequence watermarks in Figure \ref{fig:sequence_scaling}(a).

% because it is seen less often during training
% watermark decays for all models as dataset size grows larger
% trend seems to be non-linear, exploding at a certain point
% talk about both z-scores and loss
%  (results are averaged over 5 different random watermarks)
% Figure \ref{fig:sequence_scaling} shows watermark strength under scaling. In these experiments, we fix a document collection and apply a random sequence watermark. Additional details about the null distributions of the scaling experiments are in Appendix \ref{}.

% we should move this to future work?
% In designing a stealthy watermark, we will need to consider how susceptible it is to interference. When considering interference, the random character watermark is advantageous, as multiple rightholders can watermark the data while maintaining the watermark's strength. For future work, it may be possible to design a stealthy watermarking method that has a null distribution consisting of a large space of sequences that do not interfere with each other, using techniques such as paraphrasing. Another possible solution to interference is through collaborative watermarking. Instead of each rightholder watermarking their data separately, they may consider collaborative watermarking their data with the same watermark, where they may collectively take legal action if the watermark is detected in a model audit.

% For example, BLOOM-176B \cite{Bloom_scao_2022} is a 176B parameter model trained on 366B tokens. Compared to our settings, the model size increases by a factor of  $400\times$ to $2500\times $ while the dataset only increases by a factor of $30\times$. For these reasons, it may be reasonable to expect that BLOOM will also memorize the random sequence watermark here (duplicated $256\times$). 
%However, we cannot directly generalize our results, as there is a discrepancy between the training settings of our models and BLOOM, where the batch sizes for BLOOM are $4\times$ larger than the ones used here.

% These attacks assume that no normalization is applied to the input data, and a unicode data watermark likewise assumes that model creators may not apply unicode normalization over a large, multilingual training corpus. 
% For data watermarks, stealth will be an important consideration. If malicious model creators can easily detect or erase the watermark, the hypothesis test will be unable to distinguish the included watermark, and further discussion is given in \S \ref{sec:future_work}.

\begin{itemize}
    \item Perturbation of \textit{global}: 
    % \item Perturbation of \textbf{global}:  Let $r \sim U_{global}$. Then $\pi_{global}(D, r)$ returns the list of documents $D'$ where for each $r_i$ the unicode at position $i$ in the list of 28 unicode lookalikes is {maximally substituted}\footnote{all instances of original character across all documents in $D$ is replaced by its unicode substitution} into the \underline{entire document collection} $D$ if $r_i \,= \,1$, and is not substituted at all if $r_i \, = \, 0$. 
    % each index $r_i$ specifies whether the $i$'th unicode lookalike is to be substituted into $x$ according to $\pi$.

    % For each word in the vocabulary, we map it to a new word which has its characters replaced by unicode substitutions randomly. These substitutions often break up common words into rare subwords.

    \item Perturbation of \textit{word-based}: Instead of generating a mapping dictionary that is applied to all documents in $D$ globally, $r \sim U$ is used to seed the generation of a different random mapping dictionary for each word that appears in $D$. $D_r' = \pi_{word}(D, r)$ is thus $D$ when perturbed on a word-by-word basis using $r$, where different words use different mapping dictionaries. 
    
    % \item Perturbation of \textbf{word-based}: Let $r \sim U_{word}$. Then $\pi_{word}(x, r)$ returns a document $x'$ where \underline{each word} is maximally substituted according to the $28$-lengthed vector $r[28 t:28 (t+1)]$\footnote{following standard pythonic slicing notation}, where $t$ is the rank of the word when all words are sorted by order of appearance in the list of documents $D$. 

    
\end{itemize}

where each random seed $r$ defines a distinct perturbation for a given list of documents $D$. Let $\pi: (D,r) \mapsto D_r'$

%, the choice of $\pi$ thus needs to provide perturbations that the model is likely to memorize, and the choice of $f$ should strongly reflect $\pi$'s memorization after training.  % The next sections will study the effectiveness of different instantiations of $\pi$, suitable for different contexts.

